Deep Layer Aggregation

Visual recognition requires rich representations that span levels from low to high, scales from small to large, and resolutions from fine to coarse. Even with the depth of features in a convolutional network, a layer in isolation is not enough: compounding and aggregating these representations improves inference of what and where. Architectural efforts are exploring many dimensions for network backbones, designing deeper or wider architectures, but how to best aggregate layers and blocks across a network deserves further attention. Although skip connections have been incorporated to combine layers, these connections have been "shallow" themselves, and only fuse by simple, one-step operations. We augment standard architectures with deeper aggregation to better fuse information across layers. Our deep layer aggregation structures iteratively and hierarchically merge the feature hierarchy to make networks with better accuracy and fewer parameters. Experiments across architectures and tasks show that deep layer aggregation improves recognition and resolution compared to existing branching and merging schemes. The code is at https://github.com/ucbdrive/dla.

==> CVPR 2018 Deep Layer Aggregation/tab/table_boundary.tex <==
% \begin{table*}[htb]
% \begin{floatrow}[3]
% \figurebox{\caption{Comparison on BSDS}}{\includegraphics[width=\linewidth]{fig/bsds}\label{fig:bsds}}
% \tablebox{\caption{Evaluation on BSDS~\cite{arbelaez2011contour}. $^{\dagger}$ indicates PASCAL data is used in training.}}{
%  \ra{1.2}
%  \adjustbox{max width=\linewidth}{
%  \small
% \centering
%     \begin{tabular}{l ccc}
%         Method & ODS & OIS & AP \\ \midrule
%         SE~\cite{dollar2013structured} & 0.746 & 0.767 & 0.803 \\
%         DeepEdge~\cite{bertasius2015deepedge} & 0.753 & 0.772 & 0.807 \\
%         DeepContour~\cite{shen2015deepcontour} & 0.756 &  0.773 & 0.797 \\
%         %HED~\cite{xie2015holistically} (old) & 0.782 & 0.804 & 0.833 \\
%         HED~\cite{xie2015holistically} & 0.788 & 0.808 & 0.840 \\
%         CEDN~\cite{yang2016object}$^{\dagger}$ & 0.788 & 0.804 & 0.821 \\
%         UberNet~\cite{kokkinos2016ubernet} (1-Task)$^{\dagger}$ & 0.791 & 0.809 & {\bf 0.849} \\ \midrule
%         DLA-34 8s & 0.760 & 0.772 & 0.739 \\
%         DLA-34 4s & 0.767 & 0.778 & 0.751 \\
%         DLA-34 2s & 0.794 & 0.808 & 0.787 \\
%         %DLA-60 & 0.800 & 0.812 & 0.779 \\
%         DLA-102 2s & {\bf 0.803} & {\bf 0.813} & 0.781 \\
%         % DLA-169 & {\bf 0.803} & {\bf 0.813} & 0.768 \\ \hline
%     \midrule
%     \end{tabular}
%     }
%     \label{tab:edge-bsds}
% }
% \tablebox{\caption{Evaluation on Pascal Boundaries~\cite{premachandran2017pascal}.}}{
%   \ra{1.2}
%   \adjustbox{max width=\linewidth}{
%   \small
%   \centering
%     \begin{tabular}{lcccc}
%         Method & Train & ODS & OIS & AP \\ \midrule
%         SE~\cite{dollar2013structured} & \multirow{6}{*}{BSDS} & 0.541 & 0.570  & 0.486 \\
%         HED~\cite{yang2016object} & &  0.553 & 0.585 & 0.518 \\
%         DLA-34 2s & & 0.642 & 0.668 & 0.624 \\
%         DLA-102 2s & & 0.648 & 0.674 & 0.623 \\
%         \midrule
%         DSBD~\cite{premachandran2017pascal} & \multirow{6}{*}{PASCAL} & 0.643 & 0.663 & 0.650 \\
%         M-DSBD~\cite{premachandran2017pascal} & & 0.652 & 0.678 & 0.674 \\
%         DLA-34 2s & & 0.743 & 0.757 & {\bf 0.763} \\
%         DLA-102 2s & & {\bf 0.754} & {\bf 0.766} & 0.752 \\
%         \midrule
%     \end{tabular}}
% \label{tab:edge-pascal}
% }
% \end{floatrow}
% \end{table*}

\begin{table}[htp]
    \centering
    \begin{tabular}{l ccc}
        Method & ODS & OIS & AP \\ \midrule
        SE~\cite{dollar2013structured} & 0.746 & 0.767 & 0.803 \\
        DeepEdge~\cite{bertasius2015deepedge} & 0.753 & 0.772 & 0.807 \\
        DeepContour~\cite{shen2015deepcontour} & 0.756 &  0.773 & 0.797 \\
        %HED~\cite{xie2015holistically} (old) & 0.782 & 0.804 & 0.833 \\
        HED~\cite{xie2015holistically} & 0.788 & 0.808 & 0.840 \\
        CEDN~\cite{yang2016object}$^{\dagger}$ & 0.788 & 0.804 & 0.821 \\
        UberNet~\cite{kokkinos2016ubernet} (1-Task)$^{\dagger}$ & 0.791 & 0.809 & {\bf 0.849} \\ \midrule
        DLA-34 8s & 0.760 & 0.772 & 0.739 \\
        DLA-34 4s & 0.767 & 0.778 & 0.751 \\
        DLA-34 2s & 0.794 & 0.808 & 0.787 \\
        %DLA-60 & 0.800 & 0.812 & 0.779 \\
        DLA-102 2s & {\bf 0.803} & {\bf 0.813} & 0.781 \\
        % DLA-169 & {\bf 0.803} & {\bf 0.813} & 0.768 \\ \hline
    \midrule
    \end{tabular}
    \caption{
    Evaluation on BSDS ($^{\dagger}$ indicates outside data).
    ODS and OIS are state-of-the-art, but AP suffers due to recall.
    %See Figure~\ref{fig:bsds}.
    }
        % \vspace{-4mm}
    \label{tab:edge-bsds}
\end{table}

\begin{table}[htp]
    \centering
    \begin{tabular}{lcccc}
        Method & Train & ODS & OIS & AP \\ \midrule
        SE~\cite{dollar2013structured} & \multirow{4}{*}{BSDS} & 0.541 & 0.570  & 0.486 \\
        HED~\cite{yang2016object} & &  0.553 & 0.585 & 0.518 \\
        DLA-34 2s & & 0.642 & 0.668 & 0.624 \\
        DLA-102 2s & & 0.648 & 0.674 & 0.623 \\
        \midrule
        DSBD~\cite{premachandran2017pascal} & \multirow{4}{*}{PASCAL} & 0.643 & 0.663 & 0.650 \\
        M-DSBD~\cite{premachandran2017pascal} & & 0.652 & 0.678 & 0.674 \\
        DLA-34 2s & & 0.743 & 0.757 & {\bf 0.763} \\
        DLA-102 2s & & {\bf 0.754} & {\bf 0.766} & 0.752 \\
        \midrule
    \end{tabular}
    \caption{
    Evaluation on PASCAL Boundaries.
    DLA is state-of-the-art.
    }
    \label{tab:edge-pascal}
\end{table}

==> CVPR 2018 Deep Layer Aggregation/tab/table_finegrained.tex <==
% \begin{table}[ht]
%   \centering
%   \ra{1.2}
%   \adjustbox{max width=\columnwidth}{
%   \small
% 		\begin{tabular}{l c c c}
% 			%\hline
% 			 & \#Class & \#Train (per class) & \#Test (per class) \\
% 			\hline %\midrule
% 			%Bird\citep{wah2011caltech}& 200 & 5994 & 5794 & 30 \\
%             Bird& 200 & 5994 (30) & 5794 (29) \\
%             %\hline
%             %Car\citep{krause20133d} & 196 & 8144 & 8041 & 42 \\
%             Car & 196 & 8144 (42) & 8041 (41) \\
%             %\hline
% 			%Plane\citep{maji2013fine}& 102 & 6667 & 3333 & 65\\
%             Plane & 102 & 6667 (67) & 3333 (33)\\
%             %\hline
%             %Food\citep{bossard2014food} & 101 & 75750 & 25250 & 750 \\
%             Food & 101 & 75750 (750) & 25250 (250) \\
%             %\hline
%             %CompCars\citep{yang2015large}& 431 & 16016 & 14939 & 37\\
%             %\hline
% 			%NABirds\citep{van2015building}& 555 & 23929 & 24633 & 43 \\
%             %NABirds& 555 & 23929 (43) & 24633 (44) \\
% 			\hline %\midrule
%             ILSVRC & 1000 & 1,281,167 (1281) & 100,000 (100) \\
%             \hline 
% 		\end{tabular}}
% 	%\vspace{3mm}
% 	\caption{Statistic for fine-grained categorization datasets. Compared to large-scale generic classification datasets, they contain more fine-grained categories with fewer training samples. }
% 	\label{tab:fine_grained_datasets}
% 	%\vspace{-3mm}
% \end{table}

% \begin{figure*}[htb]
% 	\centering
% 	\includegraphics[width=\linewidth]{tab/fig-fine-grained.pdf}
%     % \includegraphics[width=\columnwidth]{tab/fig_finegrained.png}
% 	\caption{Comparison with state-of-the-art methods on fine-grained datasets. Image classification accuracy on Bird~\cite{wah2011caltech}, Car~\cite{krause20133d}, Plane~\cite{maji2013fine}, and Food~\cite{bossard2014food}. Higher is better. $P$ is the number of parameters in each model. For fair comparison, we calculate the number of parameters for $1000$-way classification. V- and R- indicate the base model as VGGNet-16 and ResNet-50, respectively. The numbers of Baseline, Compact \cite{gao2016compact} and Kernel \cite{cui2017kernel} are directly cited from \cite{cui2017kernel}.}
% \label{fig:fine_grained}
% \end{figure*}

\begin{figure*}[htb]
	\centering
	\includegraphics[width=\linewidth]{fig/fig-fine-grained.pdf}
    % \includegraphics[width=\columnwidth]{tab/fig_finegrained.png}
	\caption{Comparison with state-of-the-art methods on fine-grained datasets. Image classification accuracy on Bird~\cite{wah2011caltech}, Car~\cite{krause20133d}, Plane~\cite{maji2013fine}, and Food~\cite{bossard2014food}. Higher is better. $P$ is the number of parameters in each model. For fair comparison, we calculate the number of parameters for $1000$-way classification. V- and R- indicate the base model as VGGNet-16 and ResNet-50, respectively. The numbers of Baseline, Compact \cite{gao2016compact} and Kernel \cite{cui2017kernel} are directly cited from \cite{cui2017kernel}.}
\label{fig:fine_grained}
\end{figure*}

% \begin{table}[htb]
%   \centering
%   \ra{1.2}
%   \adjustbox{max width=\linewidth}{
%   \small
% \begin{tabular}{l  c  c  c  c  c  r}
% & Bird & Car & Plane & Food & P \\ \hline
% DLA-X-60-C  & 80.5 & 91.0 & 88.7 & 86.7 &  \\
% DLA-34  & 82.7 & 92.5 & 91.6 & 87.8 &  \\
% DLA-60 & 84.4 & 94.0 & 92.4 & 89.6 & \\
% DLA-X-60 & 85.0 & 93.9 & \textbf{92.9} & \textbf{90.0} & \\
% DLA-102 & \textbf{85.1} & \textbf{94.1} & 92.6 & 89.7 & \\
% % 102v75 &  &  &  &  &  & \\
% % 102v76 &  &  &  &  &  & \\
% % 169v71 &  &  &  &  &  & \\
% \midrule
% V-16-Baseline & 73.1 & 79.8 & 74.1 & 81.2 & 138.3M \\
% V-16-Compact & 84.3 & 91.2 & 84.1 & 82.4 & 18.8M\\
% V-16-Kernel & \textbf{86.2} & \textbf{92.4} & \textbf{86.9} & 84.2 & 18.8M \\
% R-50-Baseline & 78.4 & 84.7 & 79.2 & 82.1 & 25.6M \\
% R-50-Compact & 81.6 & 88.6 & 81.6 & 83.2 & 25.6M\\
% R-50-Kernel & 84.7 & 92.7 & 85.7 & \textbf{85.5} & 25.6M \\
% \hline 
% \end{tabular}}
% % \vspace{-1mm}
% \caption{Comparison with state-of-the-art methods on fine-grained datasets. Image classification accuracy on Birds~\cite{wah2011caltech}, Car~\cite{krause20133d}, Plane~\cite{maji2013fine}, and Food~\cite{bossard2014food}. Higher is better. $P$ is the number of parameters in each model. For fair comparison, we calculate the number of parameters for $1000$-way classification. V- and R- indicate the base model as VGGNet-16 and ResNet-50, respectively. The numbers of Baseline, Compact \cite{gao2016compact} and Kernel \cite{cui2017kernel} are directly cited from \cite{cui2017kernel}.}
% \label{tab:fine_grained}
% %\vspace{-2mm}
% \end{table}

% \begin{table}[htb]
%   \centering
%   \ra{1.2}
%   \adjustbox{max width=\linewidth}{
%   \small
% \begin{tabular}{l  c  c  c  c  c  r}
% %\toprule
% %Model & \tiny\citep{wah2011caltech} & \tiny\citep{krause20133d} & \tiny\citep{maji2013fine} & \tiny\citep{bossard2014food} & \tiny\citep{van2015building} & Parameter \\ \hline
%             & Bird & Car & Plane & Food & NABirds & P \\ \hline
% DLA-48-B-s  & 76.4 & 88.1 & 86.5 & 82.4 & 72.7 & 1.3M \\
% DLA-62-S-s  & 79.2 & 91.2 & 88.4 & 83.6 & 76.5 & 1.3M \\
% DLA-48-B-m & 79.4 & 91.6 & 88.0 & 84.5 & 77.1 & 4.5M \\
% DLA-36 & 82.1 & 93.0 & 90.4 & 84.9 & 81.0 & 15.8M \\
% %SSNet-62 (70m) 10 & 83.6 & 93.7 & 91.6 & 88.3 & & 17.7M\\
% DLA-62-B & 82.8 & 93.4 & 90.8 & 86.9 & 81.6 & 22.3M\\
% DLA-62-S & 83.5 & 93.6 & 91.2 & 87.7 & 83.0 & 17.7M \\
% %ResNet-50 (103m) & 80.6 & 91.5 & 88.5 & & 80.7 & 25.6M \\
% \midrule
% V-Baseline & 73.1 & 79.8 & 74.1 & 81.2 & 73.0 & 138.3M \\
% V-\cite{gao2016compact} & 84.3 & 91.2 & 84.1 & 82.4 & - & 18.8M\\
% V-\cite{cui2017kernel} & 86.2 & 92.4 & 86.9 & 84.2 & - & 18.8M \\
% R-Baseline & 78.4 & 84.7 & 79.2 & 82.1 & 80.7 & 25.6M \\
% R-\cite{gao2016compact} & 81.6 & 88.6 & 81.6 & 83.2 & - & 25.6M\\
% R-\cite{cui2017kernel} & 84.7 & 92.7 & 85.7 & 85.5 & - & 25.6M \\
% %SSNet-48 (5m)  & 74.6 & 86.3 & 83.6 & 81.7 & 72.7 & 1.3M \\
% %SSNet-62 (5m)  & 77.8 & 90.0 & 85.9 & 83.1 & 76.5 & 1.3M \\
% %SSNet-48 (18m) & 78.0 & 90.5 & 85.5 & 83.7 & 77.1 & 4.5M \\
% %SSNet-36 (60m) & 81.0 & 92.0 & 88.4 & 84.1 & 81.0 & 15.8M \\
% %SSNet-62 (70m) & 81.7 & 92.8 & 89.7 & 86.8 & 83.0 & 17.7M \\
% %SSNet-62 (90m) & 81.7 & 92.7 &  &  & 81.6 & 22.3M\\
% %ResNet-50 (103m) & 80.6 & 91.5 & 88.5 & & 80.7 & 25.6M \\
% %\midrule
% %V-Baseline & 73.1 & 79.8 & 74.1 & 81.2 & & 138.3M \\
% %V-\cite{gao2016compact} & 84.3 & 91.2 & 84.1 & 82.4 & - & 18.8M\\
% %V-\cite{cui2017kernel} & 86.2 & 92.4 & 86.9 & 84.2 & - & 18.8M \\
% %R-Baseline & 78.4 & 84.7 & 79.2 & 82.1 & & 25.6M \\
% %R-\cite{gao2016compact} & 81.6 & 88.6 & 81.6 & 83.2 & - & 25.6M\\
% %R-\cite{cui2017kernel} & 84.7 & 91.1 & 85.7 & 85.5 & - & 25.6M \\
% %\midrule
% %Others & & & & & & N/A \\
% %DRN-C-42\cite{yu2017dilated} & 81.6 & 31.2M \\
% %*VGGNet-16\cite{simonyan2015very}(need to re-run) & 73.1 & 130M \\ 
% %\bottomrule
% \hline 
% \end{tabular}}
% % \vspace{-1mm}
% \caption{Comparison with state-of-the-art methods on fine-grained datasets. Image classification accuracy on Birds~\cite{wah2011caltech}, Car~\cite{krause20133d}, Plane~\cite{maji2013fine}, Food~\cite{bossard2014food}, and NABirds~\cite{van2015building}. Higher is better. $P$ is the number of parameters in each model. For fair comparison, we calculate the number of parameters for $1000$-way classification. V- and R- indicate the base model as VGGNet-16 and ResNet-50, respectively. }
% \label{tab:fine_grained}
% %\vspace{-2mm}
% \end{table}
% \begin{table}[htb]
% \centering
% \begin{tabular}{c | l |  c  c | r}
% Dataset & Model & Accuracy & P \\ \hline
% \multirow{5}{20mm}{\centering \citep{wah2011caltech}} & SSNet-48 (5m) & 74.6 & 1.3M \\
% & SSNet-48 (18m) & 78.0 & 4.5M \\
% & SSNet-62 (5m)& 77.8 & 1.3M \\
% & SSNet-36 (60m)& 81.0 & 15.8M \\
% & SSNet-62 (70m) & 81.7 & \\
% &  SSNet-62 (90m) & 81.7 & \\
% & ResNet-50\cite{he2016deep}(need to re-run) & 78.4 & 25.6M \\
% %&\cite{krause2015fine} & 82.0 & \\
% &\cite{gao2016compact} & 84.3 & 130M\\
% &\cite{cui2017kernel} & 86.2 & 130M \\
% %DRN-C-42\cite{yu2017dilated} & 81.6 & 31.2M \\
% %*VGGNet-16\cite{simonyan2015very}(need to re-run) & 73.1 & 130M \\ 
% \midrule
% \multirow{8}{20mm}{\centering \citep{van2015building}} & AlexNet \cite{van2015building} & 35.7 & 62.4M\\
% &AlexNet+Parts\cite{van2015building} & 75.0 & 3*62.4M \\
% &SSNet-48 (5m) & 72.7 & 1.3M \\
% &SSNet-62 (5m) & 76.5 & 1.3M \\
% &SSNet-48 (18m) & 77.1 & 4.5M \\
% &SSNet-36 (60m) & 81.0 & 15.8M \\
% &SSNet-62 (70m) & 83.0 & \\
% &SSNet-62 (90m) &  & \\
% &ResNet-50\cite{he2016deep}(need to re-run) &  & 25.6M \\
% \midrule
% \multirow{6}{20mm}{\centering \citep{krause20133d}}&SSNet-48 (5m) & 86.3 & 1.3M \\
% &SSNet-48 (18m) & 90.5 & 4.5M \\
% &SSNet-62 (5m) & & 1.3M \\
% &SSNet-36 (60m)& 92.0 & 15.8M \\
% &SSNet-62 (70m) & 92.8 & \\
% &SSNet-62 (90m) & 92.7 & \\
% &ResNet-50\cite{he2016deep}(need to re-run) & 84.7 & 25.6M \\
% &\cite{gao2016compact} & 91.2 & 130M \\
% &\cite{cui2017kernel} & 92.4 & 130M \\
% \midrule
% %\multirow{6}{20mm}{\centering CompCars\cite{yang2015large}}&SSNet-48 (5m) &  & 1.3M \\
% %&SSNet-48 (18m) &  & 4.5M \\
% %&SSNet-62 (5m) & & 1.3M \\
% %&SSNet-36 (60m)&  & 15.8M \\
% %&SSNet-62 (70m) &  & \\
% %%SSNet-62 (90m) &  & \\
% %&AlexNet\cite{yang2015large} & 81.9 & 62.4M \\
% %&ResNet-50\cite{he2016deep}(need to re-run) &  & 25.6M \\
% %&GoogLeNet\cite{szegedy2015going} & 91.2 & 8.0M & 
% %\midrule
% \multirow{6}{20mm}{\centering \citep{maji2013fine}}&SSNet-48 (5m) &  & 1.3M \\
% &SSNet-48 (18m) &  & 4.5M \\
% &SSNet-62 (5m) & & 1.3M \\
% &SSNet-36 (60m)&  & 15.8M \\
% &SSNet-62 (70m) &  & \\
% &SSNet-62 (90m) &  & \\
% %SSNet-62 (90m) &  & \\
% &ResNet-50\cite{he2016deep}(need to re-run) & 79.2 & 25.6M \\
% &\cite{gao2016compact} & 84.1 & 130M \\
% &\cite{cui2017kernel} & 86.9 & 130M \\
% \midrule
% \multirow{6}{20mm}{\centering \citep{bossard2014food}}&SSNet-48 (5m) &  & 1.3M \\
% &SSNet-48 (18m) &  & 4.5M \\
% &SSNet-62 (5m) & & 1.3M \\
% &SSNet-36 (60m)&  & 15.8M \\
% &SSNet-62 (70m) &  & \\
% &SSNet-62 (90m) &  & \\
% %SSNet-62 (90m) &  & \\
% &ResNet-50\cite{he2016deep}(need to re-run) & 82.1 & 25.6M \\
% &\cite{gao2016compact} & 82.4 & 130M \\
% &\cite{cui2017kernel} & 85.5 & 25.6M \\
% %*VGGNet-16\cite{simonyan2015very}(need to re-run) & 79.8 & 130M 
% \end{tabular}
% % \vspace{-1mm}
% \caption{\dq{P for 1000-way classification}Comparison with VGG16, ResNet50 (*Comparison: https://vision.cornell.edu/se3/wp-content/uploads/2017/04/cui2017cvpr.pdf). Fine-grained classification accuracy (error rates) on the CUB-200-2011 and NABirds test set. Higher is better. $P$ is the number of parameters in each model.}
% \label{tab:fine_grained}
% %\vspace{-2mm}
% \end{table}

==> CVPR 2018 Deep Layer Aggregation/tab/table_imagenet.tex <==
% \begin{table*}[htb]
% \begin{floatrow}[2]
% \tablebox{\caption{Comparison with ResNet and ResNeXt (outdated)}}{
%  \ra{1.2}
%  \adjustbox{max width=\linewidth}{
%  \small
% \begin{tabular}{l  c  c  c}
% & Top-1 & Top-5 & P \\ \hline
% ResNet-34 & 26.0 & 8.4 & 21.8M \\
% DLA-36 & 25.1 & 7.8 & 15.8M \\
% ResNet-50 & 23.8 & 7.1 & 25.6M \\
% DLA-62-B & 22.8 & 6.4 & 22.3M \\
% ResNet-101 & 22.5 & 6.3 & 44.5M \\
% DLA-104-B & 22.0 & 6.0 & 33.7M \\
% % ResNet-152 & & & 61.2M \\
% % SSNet-160 & 21.5 & 5.8 & 53.8M  \\
% \hline
% ResNeXt-50 & 22.2 & - & 25.0M \\
% DLA-62-S & 22.2 & 6.2 & 17.7M \\
% DLA-104-S & 21.4 & 5.8 & 26.8M \\
% ResNeXt-101 & 21.2 & 5.6 & 44.0M \\
% \hline 
% \end{tabular}}
% \label{tab:resnet}
% \label{tab:resnext}
% }
% \tablebox{\caption{Comparison with compact models.}}{
%   \ra{1.2}
%   \adjustbox{max width=\linewidth}{
%   \small
% \begin{tabular}{l  c  c  c c}
%  & Top-1 & Top-5 & P & Multi-Add \\ \hline
% SqueezNet-A & 42.5 & 19.7 & 1.2M & 1.70B \\
% SqueezNet-B & 39.6 & 17.5 & 1.2M & 0.72B\\
% %% MobileNet & 39.8 & - & 1.3M & \\ \hline
% % ResNet-42-s & 40.3 & 17.4 & 1.0M & \\
% % ResNet-54-s & 37.5 & 15.5 & 1.3M & \\ \hline
% DLA-46-C & 36.8 & 15.0 & 1.3M & 0.58B\\
% DLA-46-C & 34.0 & 13.7 & 1.1M & 0.53B\\
% DLA-X-60-C & 32.5 & 12.0 & 1.3M & 0.59B\\
% \hline 
% \end{tabular}}
% \label{tab:small_model}
% }
% \end{floatrow}
% \end{table*}

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=\linewidth]{tab/fig-imagenet-params.pdf}
%     % \includegraphics[width=\linewidth]{tab/fig-imagenet.pdf}
%     % \begin{subfigure}{0.4\textwidth}
%     % % \includegraphics[width=\linewidth]{fig/imagenet_params}
%     % \includegraphics[width=\linewidth]{tab/fig-imagenet-params.pdf}
%     % \end{subfigure}
%     %     \begin{subfigure}{0.4\textwidth}
%     % \includegraphics[width=\linewidth]{tab/fig-imagenet-multiadd.pdf}
%     % %  \includegraphics[width=\linewidth]{fig/imagenet_gflops}
%     %      \end{subfigure}

%     \caption{Comparison of DLA with standard networks in terms of parameter efficiency on ILSVRC}
%     \label{fig:imagenet_params}
% \end{figure}

    \begin{figure*}[htp]
        \centering
        \includegraphics[width=\linewidth]{fig/fig-imagenet.pdf}
        % \includegraphics[width=\linewidth]{tab/fig-imagenet.pdf}
        % \begin{subfigure}{0.4\textwidth}
        % % \includegraphics[width=\linewidth]{fig/imagenet_params}
        % \includegraphics[width=\linewidth]{tab/fig-imagenet-params.pdf}
        % \end{subfigure}
        %     \begin{subfigure}{0.4\textwidth}
        % \includegraphics[width=\linewidth]{tab/fig-imagenet-multiadd.pdf}
        % %  \includegraphics[width=\linewidth]{fig/imagenet_gflops}
        %      \end{subfigure}
    
        \caption{
        Evaluation of DLA on ILSVRC.
        DLA/DLA-X have ResNet/ResNeXt backbones respectively.
        DLA achieves the highest accuracies with fewer parameters and fewer computation.
        }
        \label{fig:imagenet_params}
    \end{figure*}


\begin{table}[htp]
%   \ra{1.2}
  \adjustbox{max width=\linewidth}{
%   \small
\begin{tabular}{l  c  c  c c}
 & Top-1 & Top-5 & Params & FMAs \\ \hline
SqueezNet-A & 42.5 & 19.7 & 1.2M & 1.70B \\
SqueezNet-B & 39.6 & 17.5 & 1.2M & 0.72B\\
%% MobileNet & 39.8 & - & 1.3M & \\ \hline
% ResNet-42-s & 40.3 & 17.4 & 1.0M & \\
% ResNet-54-s & 37.5 & 15.5 & 1.3M & \\ \hline
DLA-46-C & 35.1 & 13.3 & 1.3M & 0.58B\\
DLA-X-46-C & 34.0 & 13.0 & {\bf 1.1M} & {\bf 0.53B} \\
DLA-X-60-C & {\bf 32.0} & {\bf 11.6} & 1.3M & 0.59B\\
\hline 
\end{tabular}}
\caption{
Comparison with compact models.
DLA is more accurate at the same number of parameters while inference takes fewer operations (counted by fused multiply-adds).
}
\label{tab:small_model}
\end{table}

==> CVPR 2018 Deep Layer Aggregation/tab/table_segmentation.tex <==
%\begin{table*}[htbp]
% %\setlength{\tabcolsep}{5.3pt}
% \centering
% \ra{1.2}
% \adjustbox{max width=\linewidth}{
% \small
% \begin{tabular}{l c c c c c c c c c c c c c} %{l||c|c|c|c|c|c|c|c|c|c|c||c}
% %\begin{tabular}{@{}l@{\hspace{5mm}}*{11}{@{\hspace{2mm}}c}@{\hspace{5mm}}c@{\hspace{2mm}} c}
%    & \ver{Data Aug} & \ver{Building} & \ver{Tree} & \ver{Sky} & \ver{Car} & \ver{Sign} & \ver{Road} & \ver{Pedestrian} &
%    \ver{Fence} & \ver{Pole} & \ver{Sidewalk} & \ver{Bicyclist} & \ver{mean IoU} \\ \hline
%%ALE
%\cite{russell2009associative} & & 73.4 & 70.2 & {91.1} & 64.2 & 24.4 & 91.1 & 29.1 & 31.0 &
%13.6 & 72.4 & 28.6 & 53.6 \\
%%SuperParsing
%\cite{tighe2010superparsing} & &70.4 & 54.8 & 83.5 & 43.3 & 25.4 & 83.4 & 11.6 & 18.3
%& 5.2 & 57.4 & 8.9 & 42.0 \\
%%Liu and He
%\cite{liu2015multiclass} & & 66.8 & 66.6 & 90.1 & 62.9 & 21.4 & 85.8 & 28.0 & 17.8 &
%8.3 & 63.5 & 8.5 & 47.2 \\
%%SegNet
%\cite{badrinarayanan2015segnet} & & 68.7 & 52.0 & 87.0 & 58.5 & 13.4 & 86.2 & 25.3 & 17.9 & 16.0
%& 60.5 & 24.8 & 46.4 \\
%% DeepLab-LFOV
%\cite{chen2014semantic} & & 81.5 & 74.6 & 89.0 & 82.2 & 42.3 & {92.2} & 48.4 & 27.2 & 14.3 & {75.4} & 50.1 & 61.6 \\
%%Dilation8
%\cite{yu2016multi} & & {82.6} & {76.2} & 89.9 & {84.0} & {46.9} & {92.2} & {56.3} & {35.8} & {23.4} & 75.3 & {55.5} & {65.3} \\
%\cite{kundu2016feature} & & 84.0 & 77.2 & 91.3 & 85.6 & 49.9 & 92.5 & 59.1 & 37.6 & 16.9 & 76 & 57.2 & 66.1 \\ \hline
%
%
%DLA-34 8s & \multirow{5}{*}{No} & 83.2 & 77.2 & 91.2 & 83.6 & 48.8 & 94.3 & 58.6 & 32.0 & 27.8 & 81.1 & 55.4 & 66.7 \\
%DLA-60 8s & & 83.0 & 77.0 & 91.4 & 84.1 & 46.9 & 94.1 & 58.3 & 32.8 & 26.0 & 81.3 & 56.8 & 66.5 \\
%DLA-34 & & 83.2 & 76.4 & 92.5 & 84.6 & 52.1 & 94.4 & 61.5 & 29.4 & 35.1 & 82.0 & 57.8 & 68.1 \\
%DLA-60 & & 84.4 & 77.7 & 92.6 & 87.1 & 51.4 & 95.3 & 62.2 & 32.1 & 36.2 & 84.5 & 64.1 & 69.8 \\
%DLA-102 & & 84.9 & 78.0 & 92.5 & 86.4 & 50.8 & 94.9 & 62.8 & 45.4 & 35.7 & 83.7 & 65.8 & 71.0 \\ \hline
%DLA-60 &  \multirow{3}{*}{Yes} & 86.6 & 79.3 & 92.5 & 90.9 & 55.3 & 96.2 & 65.5 & 48.6 & 37.4 & 86.9 & 66.5 & 73.2 \\
%DLA-102 & & 86.6 & 78.8 & 92.2 & 90.3 & 57.9 & 96.5 & 66.7 & 49.6 & 38.7 & 87.9 & 66.7 & 73.8 \\
%DLA-169 & & 86.9 & 78.9 & 92.5 & 89.9 & 58.5 & 96.5 & 66.1 & 55.4 & 39.0 & 87.7 & 67.7 & 74.4 \\ \hline
%
%
% \end{tabular}
% }
% \caption{Semantic segmentation results on the CamVid dataset.}
%%  \vspace{-3mm}
% \label{tab:camvid}
%\end{table*}
%
%\begin{table*}[htbp]
%\centering
%\ra{1.2}
%\adjustbox{max width=\linewidth}{
%\small
%  \begin{tabular}{@{}l@{\hspace{5mm}}*{19}{@{\hspace{2mm}}c}@{\hspace{5mm}}c@{\hspace{2mm}} c}
%  &  \ver{Road} & \ver{Sidewalk} & \ver{Building} & \ver{Wall} &
%    \ver{Fence} & \ver{Pole} & \ver{Light} & \ver{Sign} & \ver{Vegetation} & \ver{Terrain} & \ver{Sky} & \ver{Person} & \ver{Rider}
%    & \ver{Car} & \ver{Truck} & \ver{Bus} & \ver{Train} &
%    \ver{Motorcycle} & \ver{Bicycle} & \ver{mean IoU} \\
%  \midrule
%    DLA-34 8s & 97.9 & 83.2 & 91.9 & 47.7 & 57.7 & 62.4 & 68.6 & 77.3 & 92.2 & 60.4 & 94.8 & 81.1 & 59.8 & 94.1 & 57.5 & 76.6 & 54.2 & 59.7 & 76.6 & 73.4 \\
%DLA-60 8s & 97.8 & 82.9 & 91.8 & 45.7 & 55.7 & 63.3 & 70.3 & 79.3 & 92.3 & 60.9 & 95.0 & 81.8 & 60.0 & 94.1 & 50.0 & 75.8 & 51.6 & 60.6 & 77.5 & 73.0 \\ \midrule
%DLA-34 & 98.0 & 83.5 & 92.1 & 51.0 & 56.8 & 64.9 & 69.6 & 78.5 & 92.4 & 62.9 & 95.1 & 81.5 & 59.6 & 94.5 & 59.0 & 78.4 & 57.8 & 62.9 & 76.9 & 74.5 \\
%DLA-60 & 97.9 & 83.4 & 91.7 & 40.4 & 55.7 & 65.5 & 70.8 & 79.9 & 92.4 & 60.7 & 95.1 & 82.1 & 60.2 & 94.3 & 50.1 & 77.4 & 47.2 & 61.2 & 77.9 & 72.8 \\
%DLA-102 & 98.0 & 84.3 & 92.3 & 43.2 & 56.9 & 67.2 & 71.6 & 80.9 & 92.5 & 61.4 & 94.6 & 82.7 & 61.5 & 94.5 & 60.3 & 77.7 & 53.8 & 62.2 & 78.5 & 74.4 \\
%%DLA-169 & 98.2 & 84.8 & 92.5 & 45.9 & 60.0 & 68.0 & 72.3 & 81.1 & 92.7 & 61.9 & 95.1 & 83.4 & 63.3 & 95.3 & 70.9 & 80.8 & 48.1 & 65.4 & 79.1 & 75.7 \\
%\midrule
%% DLA-34 MS & 98.2 & 84.7 & 92.5 & 54.3 & 59.5 & 65.9 & 71.1 & 79.5 & 92.7 & 64.1 & 95.3 & 82.6 & 61.8 & 94.7 & 63.3 & 83.7 & 64.6 & 64.2 & 77.6 & 76.3 \\
%% DLA-60 MS & 98.1 & 84.6 & 92.1 & 43.5 & 58.2 & 66.4 & 71.8 & 81.0 & 92.7 & 62.6 & 95.3 & 83.0 & 61.2 & 94.5 & 53.5 & 82.0 & 53.0 & 64.8 & 78.9 & 74.6 \\
%
%% DLA-102 MS & 98.5 & 85.0 & 92.5 & 47.1 & 56.7 & 66.9 & 74.4 & 78.6 & 93.6 & 71.7 & 95.1 & 85.8 & 67.4 & 95.3 & 55.8 & 63.5 & 57.8 & 68.1 & 76.1 & 76.1 \\
%% DLA-169 MS & 98.3 & 85.9 & 92.8 & 48.3 & 61.2 & 69.0 & 73.4 & 82.2 & 92.9 & 63.1 & 95.4 & 84.2 & 65.1 & 95.7 & 76.3 & 82.9 & 49.6 & 68.5 & 80.2 & 77.1 \\
%
%  \end{tabular}
%}
%\vspace{-1mm}
%  \caption{
%  Performance of DLA on the Cityscapes validation set. s8 indicates the input image is downsampled by 8 in the model output. It is 2 by default. Lower downsampling rate usually leads to higher accuracy. We also find that DLA-34 has very good performance despite its smaller number of layers. 
%  % MS means multi-scale testing.
%  % Method marked with $\dagger$ used IDA to upsample the prediction results, while the other methods use bilinear interpolation to upsample the feature maps that are 8$\times$ smaller than input images in spatial resolution.
%  % The additional parameters for IDA upsampling is negligible.
%  % DRN-26 and DRN-42 are in DRN-C family proposed by \cite{yu2017dilated}}
%  % TODO scope these results: no context models, no ensembles, etc. [ES]
%  }
%\label{tab:cityscapes}
%\end{table*}
%
%\begin{table}[htp]
%    \centering
%    \begin{tabular}{cc}
%        Method & mIoU \\ \midrule
%        FCN-8s & 65.3 \\
%        RefineNet-101 & 73.6 \\
%        DLA-102 & 75.3 \\
%        DLA-169 & 75.9 \\ \midrule
%    \end{tabular}
%    \caption{Comparison on Cityscapes test set.}
%    \label{tab:city_test}
%\end{table}





\begin{table*}[htb]
\begin{floatrow}[2]
\tablebox{\caption{
Evaluation on Cityscapes to compare strides on validation and to compare against existing methods on test.
DLA is the best-in-class among methods in the same setting.
%We also find that DLA-34 has very good performance despite its smaller number of layers.
}}{
%  \ra{1.2}
 \adjustbox{max width=\linewidth}{
%  \small
    \begin{tabular}{ccc}
        Method & Split & mIoU \\ \hline
        DLA-34 8s & \multirow{3}{*}{Val} & 73.5 \\
        %DLA-60 8s & & 73.0 \\
        DLA-34 2s & & 75.1 \\
        %DLA-60 2s & & 72.8 \\
        DLA-102 2s & & 74.4 \\
        \hline
        FCN-8s \cite{shelhamer2016fully} & \multirow{4}{*}{Test} & 65.3 \\
        RefineNet-101 \cite{lin2016refinenet} & & 73.6 \\
        DLA-102 & & 75.3 \\
        DLA-169 & & {\bf 75.9} \\ \hline
    \end{tabular}}
\label{tab:cityscapes}
}
% \tablebox{\caption{Performance of DLA on the Cityscapes test set.}}{
%  \ra{1.2}
%  \adjustbox{max width=\linewidth}{
%  \small
%     \begin{tabular}{cc}
%         Method & mIoU \\ \hline
%         FCN-8s & 65.3 \\
%         RefineNet-101 & 73.6 \\
%         DLA-102 & 75.3 \\
%         DLA-169 & 75.9 \\ \hline
%     \end{tabular}}
% \label{tab:cityscapes}
% }
\tablebox{\caption{
Evaluation on CamVid.
Higher depth and resolution help.
DLA is state-of-the-art.
}}{
%   \ra{1.2}
  \adjustbox{max width=\linewidth}{
%   \small
\begin{tabular}{cc}
        %Method & Data Aug & mIoU \\ \hline
        %DLA-34 8s & \multirow{5}{*}{No} & 66.7 \\
        %%DLA-60 8s & & 66.5 \\
        %DLA-34 & & 68.5 \\
        %%DLA-60 & & 69.8 \\
        %DLA-102 & & 71.0 \\
        %\hline \hline
        %%DLA-60 & \multirow{3}{*}{Yes} & 73.2 \\
        %DLA-102 & & 73.8 \\
        %DLA-169 & & 74.4 \\ \hline
        Method & mIoU \\ \hline
        SegNet \cite{badrinarayanan2015segnet} & 46.4 \\
        DeepLab-LFOV \cite{chen2014semantic} & 61.6 \\
        Dilation8 \cite{yu2016multi} & 65.3 \\
        FSO \cite{kundu2016feature} & 66.1 \\ \hline
        DLA-34 8s & 66.7 \\
        %DLA-60 8s & & 66.5 \\
        DLA-34 2s & 68.6 \\
        %DLA-60 & & 69.8 \\
        DLA-102 2s & {\bf 71.0} \\ \hline
    \end{tabular}}
\label{tab:camvid}
}
\end{floatrow}
\end{table*}

%% SegNet
%\cite{badrinarayanan2015segnet} & & 46.4 \\
%% DeepLab-LFOV
%\cite{chen2014semantic} & & 61.6 \\
%%Dilation8
%\cite{yu2016multi} & & 65.3 \\
%\cite{kundu2016feature} & & 66.1 \\ \hline

% DLA-34 8s & \multirow{5}{*}{No} & 83.2 & 77.2 & 91.2 & 83.6 & 48.8 & 94.3 & 58.6 & 32.0 & 27.8 & 81.1 & 55.4 & 66.7 \\
% DLA-60 8s & & 83.0 & 77.0 & 91.4 & 84.1 & 46.9 & 94.1 & 58.3 & 32.8 & 26.0 & 81.3 & 56.8 & 66.5 \\
% DLA-34 & & 83.2 & 76.4 & 92.5 & 84.6 & 52.1 & 94.4 & 61.5 & 29.4 & 35.1 & 82.0 & 57.8 & 68.1 \\
% DLA-60 & & 84.4 & 77.7 & 92.6 & 87.1 & 51.4 & 95.3 & 62.2 & 32.1 & 36.2 & 84.5 & 64.1 & 69.8 \\
% DLA-102 & & 84.9 & 78.0 & 92.5 & 86.4 & 50.8 & 94.9 & 62.8 & 45.4 & 35.7 & 83.7 & 65.8 & 71.0 \\ \hline
% DLA-60 &  \multirow{3}{*}{Yes} & 86.6 & 79.3 & 92.5 & 90.9 & 55.3 & 96.2 & 65.5 & 48.6 & 37.4 & 86.9 & 66.5 & 73.2 \\
% DLA-102 & & 86.6 & 78.8 & 92.2 & 90.3 & 57.9 & 96.5 & 66.7 & 49.6 & 38.7 & 87.9 & 66.7 & 73.8 \\
% DLA-169 & & 86.9 & 78.9 & 92.5 & 89.9 & 58.5 & 96.5 & 66.1 & 55.4 & 39.0 & 87.7 & 67.7 & 74.4 \\ \hline
